Vision Transformers are Parameter-Efficient Audio-Visual Learners

Vision transformers (ViTs) have achieved impressive results on various computer vision tasks in the last several years. In this work, we study the capability of frozen ViTs, pretrained only on visual data, to generalize to audio-visual data without finetuning any of its original parameters. To do so, we propose a latent audio-visual hybrid (LAVISH) adapter that adapts pretrained ViTs to audio-visual tasks by injecting a small number of trainable parameters into every layer of a frozen ViT. To efficiently fuse visual and audio cues, our LAVISH adapter uses a small set of latent tokens, which form an attention bottleneck, thus, eliminating the quadratic cost of standard cross-attention. Compared to the existing modality-specific audio-visual methods, our approach achieves competitive or even better performance on various audio-visual tasks while using fewer tunable parameters and without relying on costly audio pretraining or external audio encoders. Our code is available at https://genjib.github.io/project_page/LAVISH/

==> figure/att_func.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.95\linewidth]{figure/images/att.png}
 	%\vspace{-2mm}
     \caption{\textbf{Learning co-attention of audio-visual features as a cue for binaural audio prediction.} For each audio component (out of $u \times t$) in the spectorgram, we perform correlation between it and the observe visual feature, which identifies the corresponding spatial region(s) of interest. With left and right weighting functions applied, the left-right audio-visual relationship can be derived and guide the learning of left-right audio difference in our framework.}
	\label{fig:att_func}
\end{figure*}

==> figure/cIoU_curve.tex <==
\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{figure/images/curve.pdf}
 	\vspace{-2mm}
     \caption{\textbf{Success ratio under different cIoU thresholds.}
     Success ratio indicates the ratio of all instances whose cIoU scores are higher than  thresholds. Note that a larger area under the curve (AUC) indicates better performance.
     }
	\vspace{\figmargin}
	\vspace{-2mm}
	\label{fig:curve}
\end{figure}


==> figure/fig_all2.tex <==

\begin{figure}[t!]
    \centering
	\includegraphics[width=0.99\linewidth]{figure/all2.pdf}
     \caption{\textbf{Putting It All Together:} \ybc{added figure}
    }
    \vspace{\figmargin}
	\label{fig:all2}
\end{figure}


==> figure/semi.tex <==
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[h]{0.48\linewidth}
    \includegraphics[width=\linewidth]{figure/images/semi_env.pdf}
    \caption{Envelope (ENV) Distance}
    \label{fig:semi_env}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.48\linewidth}
    \includegraphics[width=\linewidth]{figure/images/semi_STFT.pdf}
    \caption{STFT Distance}
    \label{fig:semi_stft}
    \end{subfigure}%
 	%\vspace{-2mm}
     \caption{Performance comparisons in terms of ENV and STFT on FAIR-PLAY using different amount of video data with ground truth binaural audio for training. Note that the horizontal axes in both figures reflects the percentage of data with ground truth audio utilized. It can be seen that our model achieved comparable results as other fully supervised models did, while only about 60\% of labeled data were used when training our model.}
	\vspace{-5mm}
	\label{fig:semi}
\end{figure*}

==> setup/graphicspath.tex <==
\graphicspath{{figure}, {images}, {example}}


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}
